Cascading Behavior in Yelp Reviews

Social media has changed the landscape of marketing and consumer research as the adoption and promotion of businesses is becoming more and more dependent on how the customers are interacting and feeling about the business on platforms like Facebook, Twitter, Yelp etc. Social review websites like Yelp have become an important source of information about different businesses. Social influence on these online platforms can result in individuals adopting or promoting ideas and actions resulting in information cascades. Research on information cascades have been gaining popularity over the last few years but most of the research has been focused on platforms like Twitter and Facebook. Research on the adoption or promotion of product using cascades can help determine important latent patterns of social influence. In this work, we have analyzed the spread of information i.e. cascades in Yelp across different cities in Europe and North America. We have enumerated and analyzed different cascade topologies that occur in the Yelp social networks. Some of our significant findings include the presence of a significant number of cascades in Yelp reviews indicating the importance of social influence, heavy-tailed distribution of cascades and possibility to accurately predict the size of cascades on the basis of initial reviews. In addition, we have also found that the characteristics of the non-root nodes and the non-root reviews are much more important type of feature as compared to the properties of the root nodes and root reviews of the cascade. These findings can help social scientists to analyze customer behavior across different cities in a much more systematic way. Furthermore, it can also help the businesses in a city to figure out different consumer trends and hence improve their processes and offerings.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> algorithm.tex <==

\newcommand{\Let}[2]{\State #1 $\gets$ #2}

\setlength{\textfloatsep}{45pt}% Remove \textfloatsep

\begin{algorithm}[!ht]

	\SetAlgoLined %\SetAlgoNoLine
	\caption{Feature Generation Algorithm\label{algorithm}}
\BlankLine
\BlankLine

	\KwData{cdr,Call Detail Records of all users}
	\KwData{opmap,Dictionary of possible operations}
	$cdrtypes \leftarrow$ [Voice, SMS, Voice and SMS]\\
	$direction \leftarrow$ [In, Out , In plus Out]\\
	$featuresArray \leftarrow$ []\\

		\BlankLine
	\KwResult{Features}
	\hrulefill
	

	Step 1: Perform reduce by grouping only on ego
	
	\BlankLine
	\ForEach {$type$, $dir1$ in {$cdrtypes$,$direction$}}{
		
			$filteredCDR \leftarrow$ $cdr$.filter($type$,$dir1$)\\
			\ForEach {$field$ in $cdr$}{
				$groupeddata \leftarrow$ $filteredCDR$.map([$ego$]+[combinations($field$])) \\
				\ForEach {$op$ in $opmap$[$field$]}{
					$reduceddata \leftarrow$ $groupeddata$.reduce($op$)
					insert $reduceddata$ in $featuresArray$\\
					$reducedata2 \leftarrow$ $reduceddata$.map($ego$,$alters$).reduce($op$)
					insert $reduceddata2$ in $featuresArray$\\
				}	
				
			}	
	}
%	\BlankLine
	\hrulefill
\end{algorithm}


==> dfa.tex <==
The Deterministic Finite Automaton described in Section \ref{sec:dfa} is defined in part by a set of transition functions $\delta : Q \times \Sigma \rightarrow Q$ that define the legal transitions between states $Q$:

\begin{itemize}
	\item \textit{Filter}: $Q \times CDR \rightarrow CDR$ \\
				Operations filter the data on the basis of the type of communication (voice, sms) or the direction the activity (incoming, outgoing).
	\item \textit{Map}: $Q \times CDR \rightarrow (field, CDR)$\\
				Operations are similar to `group by' operations, which group the input CDR according to the value of a field in the CDR. All data are initially mapped by ego $i$, creating $N$ subsets of CDR, one corresponding to each individual.
				Other common \textit{map} criteria include alter, location, and day-of-week.
	\item \textit{Select}: $Q \times (field^*,CDR) \rightarrow (field^*,fields)$ \\
				Operations extract a field (or column) from the CDR. Common select criteria are duration, location, and a constant 1 used to count transactions.
	\item \textit{Reduce}: $Q \times (field^*, fields) \rightarrow (field^*, value)$\\
				 Operations `aggregate' a set of values into a single value. Valid operations include unique, count, average, standard deviation, radius of gyration, and entropy. Whether a \textit{reduce} operation is legal depends on the data type of the field to which it is being applied. \textit{Reduce'} is a special operation that aggregates values across all of an ego's alters, creating a feature that represents the \{average, standard deviation\} of the individual's first-degree network.
\end{itemize}	


==> discussion.tex <==
Taken in the broader context of research into the determinants of Mobile Money adoption and use, the preceding results uncover several unexpected patterns. Superficially, it is not surprising that CDR-based metrics can be used to construct classifiers that predict Mobile Money use, though to our knowledge this is the first study to publish performance metrics that can serve as benchmarks in future work in this area. However, in our analysis we were surprised to find that in a given country, the supervised model was only marginally better able to identify Active Mobile Money users (who make at least one transaction per month) than Registered Mobile Money users (who make at least one transaction ever). By contrast, our expectation was that active users, who are quite rare in all three countries, would have distinct patterns of phone use that would make them easier to detect. Since most policymakers agree that true financial inclusion requires active use, this remains an open topic for future work.%

Also interesting are the differences in performance of the same modeling approach applied in different contexts (Figure \ref{fig:accuracy}). Most striking here is the relatively poor performance in Pakistan, where the 18\% improvement over the baseline is dwarfed by the 55\% improvement over the baseline achieved in Ghana.%
\footnote{This result is also unexpected, given the evidence in Figure \ref{fig:nfi}, which indicates that Ghana and Pakistan have very similar profiles in terms of relative feature importance. If anything, this figure might lead one to suspect that Zambia would be an outlier in the analysis, since Zambia's feature profile is distinct from the other two countries.}
At face value, this finding implies that Mobile Money users in Pakistan are very similar to non-Mobile Money users, or at least that the two groups have similar patterns of mobile phone user. However, looking more carefully at the data, we believe this may also in part be an artifact of the ``one size fits all'' approach we have taken to standardizing definitions and methods across countries. In particular, there is one type of Mobile Money transaction that is extremely common in Pakistan, which allows a subscriber to add prepaid phone credit to her phone account using Mobile Money. Anecdotally, it is common practice in Pakistan for the retailers of phone credit to perform this Mobile Money transaction on behalf of the subscriber. Thus, a subscriber might appear to be using Mobile Money, though in practice she was not responsible for the transaction. This potential source of bias highlights the brittle nature of the cross-country analysis, which in its current form does not allow for country-specific adaptation.

Perhaps most importantly, our results suggest that across different countries and cultures in the developing world, no single set of behavioral features is likely to consistently predict Mobile Money adoption and use. This is most clearly evident in Figure \ref{fig:transfer}, which shows that a classifier trained in one country performs very poorly when tested in another country. But the same conclusion may also be drawn from Figure \ref{fig:nfi}, where we see that the same model, when trained in different countries, selects different features and attaches different weights to to those selected features. In results not shown, we further inspect the list of top-ranked features for each country, using both (unconditional) AUC and (conditional) normalized feature importance, and note very few features that appear consistently across countries. However, even though there may not be a ``golden'' list of features that always predict Mobile Money use, we are optimistic that more generalized insights can be extracted from one context and applied in another. In ongoing work, we are exploring methods for transfer learning that may strike this balance.

More concretely, over the past several months our partner in Ghana has been using the methods we describe to generate ``Adoption Scores'' that indicate the likelihood that any given mobile subscriber will adopt and use Mobile Money. They recently reported that when using these scores to target promotions, response rates were roughly 30\% higher than promotions targeted with traditional methods. Such estimates are notoriously unreliable and subject to many possible sources of bias, but their optimism provides an indication of the potential for this line of research. At the same time, it should be noted that if the end goal is to increase financial inclusion of the poor, further methodological innovation is needed beyond what identifies the ``low hanging fruit" subscribers whose behavior indicates that they are likely to adopt of their own volition. 


%Used in predictive model. Anecdotal evidence indicates that this may be a compelling use of the algorithm. For instance, in pilot tests over the past year, the mobile operator in Ghana has used the propensity scores from our model in multiple targeted promotional campaigns, and they indicated that response rates were roughly 30\% higher than similar campaigns launched without the propensity scores. Of course, these back-of-the-envelope estimates are no substitute for quantitative evidence, and we are currently in the process of conducting a randomized trial to carefully measure whether subscribers with high Adoption Scores are indeed more likely to adopt than their counterparts with low scores. Perhaps more interesting, we are also exploring the extent to which these Adoption Scores might be used to identify subscribers who would otherwise be ``off the radar'' of traditional marketing campaigns, and who would not be likely to adopt of their own accord. After all, if the end goal is to increase financial inclusion of the poor,  a marginal reduction in the time until adoption is less valuable than reaching someone who would otherwise be left unbanked.



==> tabs/tex_table <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
\hline
 Graph                         &   Rank karlsruhe &   Frequency karlsruhe &   Rank edinburgh &   Frequency edinburgh &   Rank montreal &   Frequency montreal &   Rank pittsburgh &   Frequency pittsburgh &   Rank charlotte &   Frequency charlotte &   Rank madison &   Frequency madison &   Rank champaign &   Frequency champaign &   Rank cleveland &   Frequency cleveland &   Rank waterloo &   Frequency waterloo &   Rank vegas &   Frequency vegas &   Rank pheonix &   Frequency pheonix \\
\hline
 \textbackslash{}includegraphics\{rank\_1.png\}  &                1 &                     7 &                1 &                   157 &               1 &                  351 &                 1 &                    467 &                1 &                   558 &              1 &                 260 &                1 &                   127 &                1 &                   101 &               1 &                  419 &            1 &              3806 &              1 &                2430 \\
 \textbackslash{}includegraphics\{rank\_2.png\}  &                2 &                     1 &                2 &                    40 &               2 &                   78 &                 2 &                     96 &                2 &                   108 &              2 &                  61 &                2 &                    18 &                2 &                     5 &               2 &                   35 &            2 &               660 &              2 &                 381 \\
 \textbackslash{}includegraphics\{rank\_3.png\}  &                0 &                     0 &                5 &                    10 &               3 &                   13 &                 5 &                     15 &                3 &                    23 &              3 &                  22 &                5 &                     3 &                4 &                     1 &               0 &                    0 &            4 &               137 &              3 &                  70 \\
 \textbackslash{}includegraphics\{rank\_4.png\}  &                0 &                     0 &                3 &                    13 &               5 &                    9 &                 3 &                     28 &                4 &                    19 &              4 &                   6 &                3 &                     6 &                3 &                     1 &               7 &                    1 &            3 &               139 &              4 &                  49 \\
 \textbackslash{}includegraphics\{rank\_5.png\}  &                0 &                     0 &                7 &                     4 &              10 &                    4 &                 6 &                     12 &                7 &                    11 &              8 &                   4 &                7 &                     2 &                0 &                     0 &               5 &                    1 &            5 &                67 &              5 &                  29 \\
 \textbackslash{}includegraphics\{rank\_6.png\}  &                0 &                     0 &                4 &                    12 &               4 &                   12 &                21 &                      3 &                5 &                    18 &              5 &                   6 &                6 &                     3 &                0 &                     0 &               3 &                    3 &            7 &                41 &              6 &                  22 \\
 \textbackslash{}includegraphics\{rank\_7.png\}  &                0 &                     0 &                6 &                     5 &               6 &                    8 &                 8 &                      7 &                6 &                    12 &              9 &                   4 &               28 &                     1 &                0 &                     0 &               0 &                    0 &            6 &                42 &              8 &                  15 \\
 \textbackslash{}includegraphics\{rank\_8.png\}  &                0 &                     0 &               15 &                     2 &               8 &                    6 &                 4 &                     16 &               14 &                     4 &             15 &                   2 &                4 &                     4 &                0 &                     0 &               0 &                    0 &            9 &                27 &              7 &                  16 \\
 \textbackslash{}includegraphics\{rank\_9.png\}  &                0 &                     0 &               39 &                     1 &               0 &                    0 &                 7 &                      7 &               12 &                     4 &              6 &                   4 &                0 &                     0 &                0 &                     0 &               0 &                    0 &            8 &                30 &             11 &                  10 \\
 \textbackslash{}includegraphics\{rank\_10.png\} &                0 &                     0 &                0 &                     0 &              12 &                    3 &                10 &                      4 &               10 &                     5 &             10 &                   3 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           10 &                20 &             12 &                   9 \\
 \textbackslash{}includegraphics\{rank\_11.png\} &                0 &                     0 &               21 &                     1 &              16 &                    2 &                14 &                      3 &               11 &                     4 &             23 &                   1 &                8 &                     2 &                0 &                     0 &               0 &                    0 &           11 &                16 &              9 &                  11 \\
 \textbackslash{}includegraphics\{rank\_12.png\} &                0 &                     0 &               13 &                     2 &              15 &                    2 &                 9 &                      6 &               20 &                     2 &              7 &                   4 &               25 &                     1 &                0 &                     0 &               0 &                    0 &           14 &                11 &             10 &                  11 \\
 \textbackslash{}includegraphics\{rank\_13.png\} &                0 &                     0 &                9 &                     3 &              19 &                    2 &                12 &                      4 &                8 &                     7 &              0 &                   0 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           12 &                11 &             14 &                   6 \\
 \textbackslash{}includegraphics\{rank\_14.png\} &                0 &                     0 &                8 &                     4 &               9 &                    5 &                17 &                      3 &               16 &                     3 &             56 &                   1 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           13 &                11 &             19 &                   4 \\
 \textbackslash{}includegraphics\{rank\_15.png\} &                0 &                     0 &               45 &                     1 &              54 &                    1 &                16 &                      3 &                9 &                     6 &             16 &                   2 &               27 &                     1 &                0 &                     0 &               0 &                    0 &           16 &                 8 &             35 &                   2 \\
 \textbackslash{}includegraphics\{rank\_16.png\} &                0 &                     0 &                0 &                     0 &               7 &                    6 &                18 &                      3 &               76 &                     1 &             58 &                   1 &                0 &                     0 &                0 &                     0 &               4 &                    2 &           27 &                 5 &             23 &                   3 \\
 \textbackslash{}includegraphics\{rank\_17.png\} &                0 &                     0 &                0 &                     0 &               0 &                    0 &                11 &                      4 &               79 &                     1 &             42 &                   1 &               20 &                     1 &                0 &                     0 &               0 &                    0 &           21 &                 7 &             15 &                   6 \\
 \textbackslash{}includegraphics\{rank\_18.png\} &                0 &                     0 &                0 &                     0 &              13 &                    3 &                26 &                      2 &               13 &                     4 &             11 &                   2 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           75 &                 2 &             24 &                   3 \\
 \textbackslash{}includegraphics\{rank\_19.png\} &                0 &                     0 &               26 &                     1 &              28 &                    1 &                 0 &                      0 &               15 &                     3 &              0 &                   0 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           35 &                 3 &             13 &                   7 \\
 \textbackslash{}includegraphics\{rank\_20.png\} &                0 &                     0 &               30 &                     1 &              55 &                    1 &                 0 &                      0 &               17 &                     2 &              0 &                   0 &                0 &                     0 &                0 &                     0 &               0 &                    0 &           19 &                 7 &             18 &                   4 \\
\hline
\end{tabular}
